Soundness of reset workflow nets

Workflow nets are a well-established variant of Petri nets for the modeling of process activities such as business processes. The standard correctness notion of workflow nets is soundness, which comes in several variants. Their decidability was shown decades ago, but their complexity was only identified recently. In this work, we are primarily interested in two popular variants: $1$-soundness and generalised soundness. Workflow nets have been extended with resets to model workflows that can, e.g., cancel actions. It has been known for a while that, for this extension, all variants of soundness, except possibly generalised soundness, are undecidable. We complete the picture by showing that generalised soundness is also undecidable for reset workflow nets. We then blur this undecidability landscape by identifying a property, coined ``$1$-in-between soundness'', which lies between $1$-soundness and generalised soundness. It reveals an unusual non-monotonic complexity behaviour: a decidable soundness property is in between two undecidable ones. This can be valuable in the algorithmic analysis of reset workflow nets, as our procedure yields an output of the form ``$1$-sound'' or ``not generalised sound'' which is always correct.

==> sec-clean-1sound.tex <==
\begin{lemma}\label{lem:clanToProperCompletion}
  Let $\W$ be a clean reset workflow net. It is the case that $\W$
  properly completes.
\end{lemma}

\begin{proof}
  Let $\m$ be a configuration reached from $\{\initial \colon n\}$ in
  $\W$. Marking $\Res{\m}$ can be reached from $\{\initial \colon n\}$
  in the cleaned skeleton of $\W$. As the cleaned skeleton is
  generalized sound (because $\W$ is clean), we conclude that if
  $\Res{\m} = \{\final \colon k\}$, then $k = n$, as required.
\end{proof}

\begin{lemma}\label{lem:cleanToTrapFree}
  It is possible to decide, given a maybe sound clean reset workflow
  net $\W$, whether $W$ is trap-free.
\end{lemma}

\begin{proof}
  Let $X'$ be a set of configurations from which it is impossible to
  cover $\{\final \colon 1\}$. We define $X \defeq X' + \set{\{\final
    \colon n\} : n \in \N}$ as the set of markings from which it is
  impossible to produce tokens in place $\final$.

  We claim that there exists $n \in \N$ such that $\{\initial \colon
  n\} \trans{\pi} X$ iff there exists $n' \in \N$ such that in the
  cleaned skeleton of $\W$, marking $\Res{X}$ is reachable form
  $\{\initial \colon n'\}$.

  The implication from left to right is simple. We take $n' \defeq n +
  z$ and the
  \[
  \{\initial \colon n + z\}
  %
  \trans{\pi}
  %
  \{\initial \colon z\} + \m
  %
  \trans{\zeta}
  %
  \{\final \colon z\} + \Res{\m}.
  \]
  The implication in the opposite direction is a direct consequence of
  \Cref{lem:OnlyMReachable}.

  Thus, first we compute $X$ using the backward coverability
  algorithm. Next, we ask about reachability of a downward-closed set
  in the cleaned skeleton of $\W$.
\end{proof}

\begin{theorem}
  It is possible to decide, given a reset workflow net $\W$, whether
  $\W$ is $1$-sound or not generalized sound.
\end{theorem}

\begin{proof}
  First, we check whether $\W$ is maybe sound and clean. If not, then
  we say that it is not generalized sound. Next, as it is clean, it
  properly completes by
  \Cref{lem:clanToProperCompletion}. Furthermore, since $\W$ is both
  clean and maybe sound, we can test whether $\W$ is trap-free by
  \Cref{lem:cleanToTrapFree}. If not, then it is not generalized
  sound. Finally, we test whether form $\{\initial \colon 1\}$ it is
  possible to strictly cover $\{\final \colon 1\}$. If so, then $\W$
  is not generalized sound. Otherwise, we invoke
  \Cref{thm:characterizationOne} and conclude that $\W$ is $1$-sound.
\end{proof}


==> sec-clean.tex <==
\begin{definition}
  The \emph{skeleton} of a reset workflow net $\W$ is the Petri net
  obtained by removing all places from $\W$ that can be reset,
  i.e.\ each place $p$ for which there is a transition that resets
  $p$. The \emph{cleaned skeleton} is obtained from the skeleton by
  removing isolated transitions.

  We say that a reset workflow net $\W$ is \emph{clean} if the
  following conditions are satisfied:
  \begin{enumerate}
  \item it is maybe sound,

  \item its cleaned skeleton is a workflow net with initial place $i$
    and final place $f$,
    
  \item the skeleton workflow net is generalized sound.
  \end{enumerate}
\end{definition}

\begin{theorem}
  Every non-redundant reset workflow net that is generalized sound is
  also clean.
\end{theorem}

\begin{proof}
  Let $\W$ be a non-redundant reset workflow net that is generalized
  sound. Let $\PN$ be its cleaned skeleton. We have to prove the
  following facts: $\PN$ is a workflow net and $\PN$ is generalized
  sound.
  %, and third that for every transition $t$ there is a run $\zeta_t$.
  The fact that $\PN$ is a workflow net is proved in
  \Cref{lem:skeletonIsAWorkflow}.

  To prove the second fact, we have to prove that for every $k \in \N$
  and every marking $\m$ reachable from $\{\initial \colon k\}$ in
  $\PN$, there is a run $\m \trans{*} \{\final \colon k\}$ in $\PN$.
  We prove this by showing that if $\{\initial \colon k\} \trans{*}
  \m$ holds in $\PN$, then there exists $k' \in \N$ such that
  $\{\initial \colon k'\} \trans{*} \m + \{\final \colon k' - k\}$ in
  $\W$. This is done in \Cref{lem:OnlyMReachable}. We finish by
  observing that if $\m \trans{*} \{\final \colon k\}$ holds in $\W$,
  then $\m \trans{*} \{\final \colon k\}$ holds in $\PN$. The latter
  is proved in \Cref{lem:EveryPlaceCanBeUnMarkedINTheSkeleton}.
  %
  % To prove the third fact we observe that if the workflow is
  % non-redundant then for every $t$ there is a $k_t\in \N$ such
  % that there is a run
  % $(\initial:k)\trans{\pi_t}\vec{m_t}\trans{t}\vec{m_t'}$
  % for some markings $\vec{m_t}$ and $\vec{m_t'}$. But $W$ is
  % generalized sound, so there is a run
  % $\vec{m_t'}\trans{\pi_t'}(\final:k_t)$. We define a run
  % $\zeta_t=\pi_t t \pi_t'$ it goes as required
  % $(\initial:k_t)\trans{\zeta_t}(\final:k_t)$ and uses the
  % transition $t$.
\end{proof}

\begin{lemma}\label{lem:skeletonIsAWorkflow}
  A cleaned skeleton $\PN$ of a generalized sound non-redundant reset
  workflow net $\W$ is a workflow net.
\end{lemma}

\begin{proof}
  Places $\initial$ and $\final$ are in $\PN$ by
  \Cref{lem:IFinSkeleton}. For every transition $t$ of $\PN$, we have
  that $\pre{t} \neq \emptyset$ and $\post{t} \neq \emptyset$. This
  follows from \Cref{lem:PrePostNotEmpty}. So, to prove that every
  node in $\PN$ lies on a path from $\initial$ to $\final$, it is
  sufficient to show that every place $p$ in $\PN$ is on a path from
  $\initial$ to $\final$. The latter is a consequence of
  \Cref{lem:PathFromItoP,lem:PathFromPtoF}.
\end{proof}

\begin{lemma}\label{lem:IFinSkeleton}
  Let $\W$ be a reset workflow net that generalized. It is the case
  that $i$ and $f$ are in its skeleton.
\end{lemma}

\begin{proof}
  We have to prove that there is no transition that resets $i$ or $f$.
  We only prove the fact that $i$ belongs to the skeleton, as the
  proof for $f$ is almost the same. For the sake of contradiction,
  suppose that $t$ is a transition that resets $i$. There exists $k
  \in \N$ such that $\{I \colon k\}$ from which $t$ can be fired,
  i.e.\ there exist a run $\pi$ and a marking $\m$ such that $\{i
  \colon k\} \trans{\pi t} \m$. Observe that $\{i \colon k+1\}
  \trans{\pi t} \m$, which is a contradiction as from $\m$ both $\{f
  \colon k\}$ and $\{k \colon k+1\}$ should be reachable.
\end{proof}

\begin{lemma}\label{lem:badconf}
  Let $\W$ be a reset workflow net and let $p$ be a place that cannot
  be reset in $\W$. Suppose that for some $k \in \N$ there are two
  runs $\{i \colon k\} \trans{\pi} \m$ and $\{i \colon k\}
  \trans{\pi'} \m'$ where $\m' \geq \m + \{p \colon 1\}$. It is the
  case that $\W$ is not generalized sound.
\end{lemma}

\begin{proof}
  We consider two cases: (i)~$\{\final \colon k\}$ is not reachable
  from $\m$, (ii)~there is a run $\m \trans{\gamma} \{\final \colon
  k\}$. In the first case, it is readily seen that $\W$ is not
  generalized sound. In the second case, we consider a run $\{\initial
  \colon k\} \trans{\pi'\gamma} \{\final \colon k, p \colon 1\} + \m'$
  where $\m'$ is some marking. This contradicts general soundness as
  well.
\end{proof}

Let $\Res{NoArg} \colon \N^{\Places} \to \N^{\Places}$ be such that
\[
(\Res{\vec{x}})(p)  =
\begin{cases}
  \m(p) & \text{if } p \text{ cannot be reset}, \\
      0 & \text{otherwise}.
\end{cases}
\]

Let $\{i \colon z\} \trans{\zeta} \{f \colon z\}$ be a run that fires
every transition. It is a concatenation of $\zeta_t$ for all
transitions $t$, while $z$ is a sum of $z_t$ (see
\Cref{def:zetaRuns}). It has the important property that for any
marking $\m$, we have $\{i \colon z\} + \m \trans{\zeta} \{f \colon
z\} + \Res{\m}$.

\begin{lemma}\label{lem:PrePostNotEmpty}
  Let $\W$ be a generalized sound reset workflow net. For every
  transition $t$ of the cleaned skeleton of $\W$, we have $\pre{t}
  \neq \emptyset$ and $\post{t} \neq \emptyset$.
\end{lemma}

\begin{proof}
  Suppose that there is a transition $t$ such that $\pre{t} =
  \emptyset$ in the cleaned skeleton. As $t$ is in the cleaned
  skeleton, there exists $p \in \post{t}$ in the cleaned skeleton. Let
  us consider the following runs:
  \begin{enumerate}
  \item $\{i \colon n\} \trans{\pi} \m \trans{t} \m_1$ (it exist as
    $\W$ is non-redundant),

  \item $\{i \colon n + z\} \trans{\pi} \m + \{i \colon z\}
    \trans{\zeta} \colon \{f \colon z\} + \Res{\m}$,

  \item $\{i \colon n + z\} \trans{\pi} \m + \{i \colon z\} \trans{t}
    \m_1 + \{i \colon z\} \trans{\zeta} \Res{\m_1} + \{f \colon z\}$.
  \end{enumerate}
  The last two runs are constructed from the first run. Observe that
  $\Res{\m_1} + \{f \colon z\} \geq \Res{\m} + \{f \colon z, p \colon
  1\}$. Indeed, $\m_1 = \m - \Rest{t}{\pre{t}} + \post{t}$, but if we
  fire $\zeta$ from this configuration, then we reset it:
  \begin{align*}
    \m_1 '
    %
    &= \Res{\m_1} \\
    %
    &= \Res{\m - \Rest{t}{\pre{t}} + \post{t}} \\
    %
    &= \Res{\m} - \Res{\pre{t}} + \Res{\post{t}} \\
    %
    &= \Res{\m} - \vec{0} + \Res{\post{t}} \\
    %
    &\geq \Res{\m} - \{p \colon 1\}.
  \end{align*}
  This contradicts \Cref{lem:badconf} as $\m' = \Res{\m}$.

  Now, suppose there is a transition $t$ such that $\post{t} =
  \emptyset$ in the cleaned skeleton. As $t$ is in the cleaned
  skeleton, there exists $p \in \pre{t}$ in the cleaned skeleton. Let
  us consider the following runs:
  \begin{enumerate}
  \item $\{i \colon n\} \trans{\pi} \m \trans{t}\m_1$ (it exist as $W$
    is non-redundant),

  \item $\{i \colon n + z\} \trans{\pi} \m + \{i \colon z\}
    \trans{\zeta} \m' + \{f \colon z\}$,

  \item $\{i \colon n + z\} \trans{\pi} \m + \{i \colon z\} \trans{t}
    \m_1 + \{i \colon z\} \trans{\zeta} \m_1' + \{f \colon z\}$.
  \end{enumerate}
  The last two runs are constructed from the first one. Observe that
  $\m_1' + \{f \colon z, p \colon 1\} \leq \m' + \{f \colon
  z\}$. Indeed, $\m_1 = \m - \Rest{t}{\pre{t}} + \post{t}$ and, if we
  fire $\trans{\zeta}$ from this configuration, then we reset it:
  \begin{align*}
    \m_1'
    %
    &= \Res{\m_1} \\
    %
    &= \Res{\m - \Rest{t}{\pre{t}} + \post{t}} \\
    %
    &= \Res{\m} - \Res{\pre{t}} + \Res{\post{t}} \\
    %
    &= \Res{\m} - \Res{\pre{t}},
  \end{align*}
  which is larger than $\Res{\m} + \{p \colon 1\}$. This contradicts
  \Cref{lem:badconf} as $\m' = \Res{\m}$.
\end{proof}

\begin{definition}
  A \emph{siphon} in a reset Petri net is a subset of places $S$ such
  that, for every transition $t$, if $\post{t} \cap S \neq \emptyset$
  then $\pre{t} \cap S \neq \emptyset$. Similarly, a \emph{trap} is a
  subset of places $S$ such that, for every transition $t$, if
  $(\pre{t} \cup \reset{t}) \cap S \neq \emptyset$, then $\post{t}
  \cap S \neq \emptyset$.
\end{definition}

\begin{lemma}\label{lem:UnmarkedSiphon}\label{lem:MarkedTrap}
  Every unmarked siphon remains unmarked and every marked trap remains
  marked.
\end{lemma}

% 
% \begin{lemma}\label{lem:theSameRun}
% Let $\pi$ be a run in the reset workflow $W$ from initial marking $\m$. Let $\m'$ be a marking in the skeleton of $W$ obtained from $\m$ by 
% removing places not present in the skeleton. Then run $\pi$ is a run from $\m'$ in the skeleton of $W$. 
% \end{lemma}
% 
% It is trivial as in skeleton has the same set of transition as $W$ and only some places (constraints) are removed.

\begin{lemma}\label{lem:PathFromItoP}
  Let $\W$ be a non-redundant generalized sound reset workflow net and
  let $\PN$ be its skeleton. For every place $p$, there is a path form
  $\initial$ to $p$ in $\PN$.
\end{lemma}

\begin{proof}
  For the sake of contradiction, suppose that there is a place $p$
  such there is no path form $\initial$ to $p$ in $\PN$. First,
  observe that place $p$ can be marked in $\PN$ due to
  \Cref{lem:EveryPlaceCanBeMarkedINTheSkeleton}.
  
  Second, let $X$ be a set of places in the skeleton from which there
  is a path to $p$. Observe that this set is a siphon in the cleaned
  skeleton, indeed if some transition $\post{t}\cap X\neq \emptyset$
  then $\pre{t}\subseteq X$ and $\pre{t}\neq \emptyset$ because of
  \Cref{lem:PrePostNotEmpty}. But, in the initial marking, $X$ is
  empty as it does not contain $\initial$. So, $p$ cannot be marked as
  every unmarked siphon remains unmarked
  (by~\Cref{lem:UnmarkedSiphon}). This contradicts non-redundancy.
\end{proof}

\begin{lemma}\label{lem:PathFromPtoF}
  Let $\W$ be a non-redundant generalized sound reset workflow net and
  let $\PN$ be its skeleton. For any place $p$ of $\PN$, there is a
  path form $p$ to $\final$ in $\PN$.
\end{lemma}

\begin{proof}
  For the sake of contradiction, suppose that there is a place $p$
  such there is not path form $p$ to $\final$ in $\PN$. First, observe
  that, by \Cref{lem:EveryPlaceCanBeUnMarkedINTheSkeleton}, there
  exist a marking $\m$ and a run such that $\m(p) > 0$ and $\m
  \trans{\pi} \{\final \colon k\}$ for some $k \in \N$.
 
  Second, let $X$ be a set of places in the skeleton to which there is
  a path from $p$. Observe that this set is a trap in $\PN$. Indeed,
  for every transition $t$, we have $\Res{t} = \emptyset$ in $\PN$ and
  hence $\pre{t} = \pre{t} \cup \reset{t}$; now, if some transition
  $\pre{t} \cap X \neq \emptyset$ then $\post{t} \subseteq X$ and
  $\post{t} \neq \emptyset$ because of \Cref{lem:PrePostNotEmpty}. But
  in the marking $\m$, the set $X$ is marked and, as it is a trap, it
  cannot be unmarked (by \Cref{lem:MarkedTrap}). Thus, from $\m$ is is
  impossible to reach a marking where $\final$ is the only marked
  place. This contradicts general soundness.
\end{proof}

\begin{lemma}\label{lem:EveryPlaceCanBeMarkedINTheSkeleton}
  Let $\W$ be a non-redundant reset workflow net. Every place $p$ in
  its cleaned skeleton can be marked.
\end{lemma}

\begin{proof}
  Every place can be marked in $\W$ as the workflow is
  non-redundant. Every place in the skeleton can be marked as the
  skeleton is produced from $\W$ by removing places. Thus, every
  sequence of transitions that can be fired in $\W$ can be also fired
  in the skeleton. In the cleaned skeleton, some transitions are
  removed but we remove only transitions that do not affect any place
  in the cleaned skeleton, so if some place can be marked in the
  skeleton, then it can be marked in the cleaned skeleton as well.
\end{proof}

\begin{lemma}\label{lem:EveryPlaceCanBeUnMarkedINTheSkeleton}
  Let be a non-redundant generalized sound reset workflow net $\W$ and
  let $p$ be a place in its cleaned skeleton. There exists $k \in \N$
  and a marking $\m$ of the workflow net $\PN$, such that $\{\initial
  \colon k\} \trans{*} \m$ where $\m(p) > 0$. Moreover, for any such
  marking $\m$, we have $\m \trans{*} \{\final \colon k\}$.
\end{lemma}

\begin{proof}
  As $\W$ is non-redundant, there is an initial marking $\{\initial
  \colon k\}$ from which there is a run to some marking $\m'$ that
  marks place $p$. The same sun can be performed in $\PN$ reaching
  $\m$, which is $\m'$ restricted to places in the skeleton. As $\W$
  is generalized sound, there is run $\m' \trans{\pi} \{\final \colon
  k\}$. In the skeleton, the sequence of transitions $\pi$ yields a
  run $\m \trans{\pi} \{\final \colon k\}$. Now, in the cleaned
  skeleton, we perform $\pi$ without isolated transitions, reaching
  the same result.
\end{proof}

\begin{lemma}\label{lem:OnlyMReachable}
  Let $\W$ be a maybe sound non-redundant reset workflow net $\W$ and
  let $\PN$ be is its cleaned skeleton (which is a workflow net). Let
  $\m$ be a marking of $\PN$ reachable from $\{\initial \colon k\}$
  for some $k \in \N$. There exists $k' \in \N$ such that $\{\initial
  \colon k'\} \trans{*} \m + \{\final \colon k' - k\}$ in $\W$.
\end{lemma}

\begin{proof}
  We proceed by induction on the length of the run from $\{\initial
  \colon k\}$ to $\m$. If the length is $0$, then the claim is trivial
  and $k' = k$.

  Suppose the induction claim holds for every marking $\m$ reachable
  via a run of length at most $i$. Let $t$ be a transition and let
  $\pi' = \pi t$ be a run of length $i + 1$ such that $\{\initial
  \colon k\} \trans{\pi} \m' \trans{t} \m$. By induction hypothesis,
  we know that there exists $k'' \in \N$ such that $\{\initial \colon
  k'' + k\} \trans{} \m' + \{\final \colon
  k''\}$. \michael{$\trans{*}$?} Thus, it is sufficient to prove that
  there exists $k_t \in \N$ such that $\{\initial \colon k_t\} + \m'
  \trans{} \m + \{\final \colon k_t\}$. \michael{$\trans{*}$?}
  Indeed, then we put $k' = k'' + k + k_t$.

  Let us recall the run $\zeta$ such that $\{\initial \colon z\}
  \trans{\zeta} \{f \colon z\}$ and it fires every transition. Since
  $\W$ is maybe sound, there is a run $\{\initial \colon z_t\}
  \trans{\rho} \m_t \trans{t} \m_t'$ where $z_t \in \N$ is given by
  \Cref{def:zetaRuns}. Let us consider the following run:
  \[
  \{\initial \colon z_t + z\}
  %
  \trans{\rho}
  %
  \m_t + \{\initial \colon z\}
  %
  \trans{\zeta}
  %
  \Res{\m_t} + \{\final \colon z\}
  %
  \trans{\rho'}
  %
  \{\final \colon z_t + z\}.
  \]
  The run $\rho'$ exists as $\W$ is maybe sound \piotr{correct
    definition of maybe soundness}. So, we have the following run:
  \begin{alignat*}{3}
    &&& \{\initial \colon z_t + z\} + \m' \\
    %
    &\trans{\rho}\ &&
    %
    \{\initial \colon z\} + \Res{\m_t} + (\m_t - \Res{\m_t}) + \m' \\
    %
    &\trans{t}\ &&
    %
    \{\initial \colon z\} + \Res{\m_t} + {} \\
    %
    &&& \Rest{t}{\m_t - \Res{\m_t} - (\pre{t} - \Res{\pre{t}})} + {} \\
    %
    &&& \m + (\post{t} - \Res{\post{t}}).
  \end{alignat*}

  The last transition works as follows. First, it consumes
  $\pre{t}$. We split in into two parts, $\Res{\pre{t}}$ and $\pre{t}
  - \Res{\pre{t}}$. The first part is consumed from $\m'$. The second
  part is written explicitly. Next, we apply $\Rest{t}{\cdot}$ but it
  does not affect $\initial$, and the places marked in $\Res{\m_t}$ as
  well as $\m' - \Res{\pre{t}}$. So, we only apply it to $\m_t -
  \Res{\m_t} - (\pre{t} - \Res{\pre{t}})$. Finally, we add $\post{t}$,
  we split it into two parts, one more time, $\Res{\post{t}}$ and
  $\post{t} - \Res{\post{t}}$. The first part is added to $\m' -
  \Res{\pre{t}} + \Res{\post{t}} = \m$, and the second part is written
  explicitly.

  Note that $\Rest{t}{\m_t - \Res{\m_t} - (\pre{t} - \Res{\pre{t}})}$
  is a proper marking as $m_t \geq \pre{t}$.\michael{What is
    ``proper''?}

  Now, we continue the run as required:
  \begin{alignat*}{3}
    &&& \{\initial \colon z\} + \Res{\vec{m_t}} + {} \\
    %
    &&& \Rest{t}{\m_t - \Res{\m_t} - (\pre{t} - \Res{\pre{t}})} + {} \\
    %
    &&& \m + (\post{t} - \Res{\post{t}}) \\
    %
    & \trans{\zeta} &&
    %
    \{\final \colon z\} + \Res{\m_t} + \vec{0} + \m + \vec{0} \\
    %
    &\trans{\rho'} &&
    %
    \{\final \colon z + z_t) + \m. \tag*{\qedhere}
  \end{alignat*}
\end{proof}

\begin{theorem}
  It is possible to test whether a workflow net is clean in
  Ackermannian time.
\end{theorem}

\begin{proof}
  First, we check whether, for every transition $t$, there exists $k
  \in \N$ such that from $\{\initial \colon k\}$ it is possible to
  cover $\pre{t}$. To do this, we use the backward coverability
  algorithm~\cite{?}. Second, for a given reset workflow $\W$, we
  construct its cleaned skeleton $\PN$ in polynomial time, and we test
  whether is a workflow net in polynomial time. Next, we check whether
  $\PN$ is generalized sound (which can be done in PSPACE
  by~\cite{?}).
\end{proof}

